reslr: An R package for relative sea level modelling

We present reslr, an R package to perform Bayesian modelling of relative sea level data. We include a variety of different statistical models previously proposed in the literature, with a unifying framework for loading data, fitting models, and summarising the results. Relative sea-level data often contain measurement error in multiple dimensions and so our package allows for these to be included in the statistical models. When plotting the output sea level curves, the focus is often on comparing rates of change, and so our package allows for computation of the derivative of sea level curves with appropriate consideration of the uncertainty. We provide a large example dataset from the Atlantic coast of North America and show some of the results that might be obtained from our package.

==> roughworkreferences.tex <==

\hypertarget{refs}{}
\leavevmode\vadjust pre{\hypertarget{PSMSLinstruction}{}}%
Aarup, T., M. Merrifield, B. Pérez Gómez, I. Vassie, and P. Woodworth. 2006. {``{Manual on Sea-level Measurements and Interpretation, Volume IV : An update to 2006.}''} \emph{Intergovernmental Oceanographic Commission of UNESCO} 4.

\leavevmode\vadjust pre{\hypertarget{Ashe2019}{}}%
Ashe, Erica L., Niamh Cahill, Carling Hay, Nicole S. Khan, Andrew Kemp, Simon E. Engelhart, Benjamin P. Horton, Andrew C. Parnell, and Robert E. Kopp. 2019. {``{Statistical modeling of rates and trends in Holocene relative sea level}.''} \emph{Quaternary Science Reviews} 204: 58--77.

\leavevmode\vadjust pre{\hypertarget{Barnett2017}{}}%
Barnett, Robert L., Pascal Bernatchez, Michelle Garneau, and Marie-Noëlle Juneau. 2017. {``Reconstructing Late {H}olocene Relative Sea-Level Changes at the {M}agdalen {I}slands ({G}ulf of {S}t. {L}awrence, {C}anada) Using Multi-Proxy Analyses.''} \emph{Journal of Quaternary Science} 32 (3): 380--95.

\leavevmode\vadjust pre{\hypertarget{deBoor1978}{}}%
Boor, Carl de. 1978. {``A {P}ractical {G}uide to {S}pline.''} \emph{Applied Mathematical Sciences, New York: Springer, 1978} 27 (January). \url{https://doi.org/10.2307/2006241}.

\leavevmode\vadjust pre{\hypertarget{Brain2012}{}}%
Brain, Matthew J., Antony J. Long, Sarah A. Woodroffe, David N. Petley, David G. Milledge, and Andrew C. Parnell. 2012. {``{Modelling the effects of sediment compaction on salt marsh reconstructions of recent sea-level rise}.''} \emph{Earth and Planetary Science Letters} 345-348: 180--93.

\leavevmode\vadjust pre{\hypertarget{Cahill2015aStats}{}}%
Cahill, Niamh, Andrew C Kemp, Benjamin P Horton, and Andrew C Parnell. 2015. {``{Modeling sea-level change using {E}rrors-in-{V}ariables integrated {G}aussian {P}rocess 1}.''} \emph{The Annals of Applied Statistics} 9 (2): 547--71. \url{https://doi.org/10.1214/15-AOAS824}.

\leavevmode\vadjust pre{\hypertarget{Cahill2016}{}}%
---------. 2016. {``A {B}ayesian Hierarchical Model for Reconstructing Relative Sea Level: From Raw Data to Rates of Change.''} \emph{Climate of the Past} 12 (2): 525--42.

\leavevmode\vadjust pre{\hypertarget{Cahill2015_cp}{}}%
Cahill, Niamh, Stefan Rahmstorf, and Andrew C Parnell. 2015. {``Change Points of Global Temperature.''} \emph{Environmental Research Letters} 10 (8): 84002.

\leavevmode\vadjust pre{\hypertarget{Dean2019}{}}%
Dean, S., Benjamin P. Horton, Niki Evelpidou, Niamh Cahill, Giorgio Spada, and Dorit Sivan. 2019. {``{Can we detect centennial sea-level variations over the last three thousand years in Israeli archaeological records?}''} \emph{Quaternary Science Reviews} 210: 125--35. https://doi.org/\url{https://doi.org/10.1016/j.quascirev.2019.02.021}.

\leavevmode\vadjust pre{\hypertarget{Dey2000}{}}%
Dey, Dipak K, Sujit K Ghosh, and Bani K Mallick. 2000. \emph{Generalized Linear Models: A {B}ayesian Perspective}. CRC Press.

\leavevmode\vadjust pre{\hypertarget{Dierckx1995}{}}%
Dierckx, Paul. 1995. \emph{Curve and Surface Fitting with Splines}. Oxford University Press.

\leavevmode\vadjust pre{\hypertarget{Donnelly2006}{}}%
Donnelly, Jeffrey P. 2006. {``{A Revised Late Holocene Sea-Level Record for Northern Massachusetts, USA}.''} \emph{Journal of Coastal Research} 22 (5): 1051--61.

\leavevmode\vadjust pre{\hypertarget{Donnelly2004}{}}%
Donnelly, Jeffrey P, Peter Cleary, Paige Newby, and Robert Ettinger. 2004. {``Coupling Instrumental and Geological Records of Sea-Level Change: Evidence from Southern {N}ew {E}ngland of an Increase in the Rate of Sea-Level Rise in the Late 19th Century.''} \emph{Geophysical Research Letters} 31 (5).

\leavevmode\vadjust pre{\hypertarget{Edwards2015_SLhandbook}{}}%
Edwards, Robin, and Alex Wright. 2015. {``Foraminifera: Handbook of Sea‐level Research.''} In, 191--217. John Wiley \& Sons, Ltd. https://doi.org/\url{https://doi.org/10.1002/9781118452547.ch13}.

\leavevmode\vadjust pre{\hypertarget{eilers_1996}{}}%
Eilers, Paul, and Brian Marx. 1996. {``{Flexible Smoothing with B-splines and Penalities}.''} \emph{Statistical Science} 11.

\leavevmode\vadjust pre{\hypertarget{Engelhart2009}{}}%
Engelhart, Simon E., Benjamin P. Horton, Bruce C. Douglas, W. Richard Peltier, and Torbjörn E. Törnqvist. 2009. {``{Spatial variability of late Holocene and 20th century sea-level rise along the Atlantic coast of the United States}.''} \emph{Geology} 37 (12): 1115--18. \url{https://doi.org/10.1130/G30360A.1}.

\leavevmode\vadjust pre{\hypertarget{Gehrels1994}{}}%
Gehrels, Roland W. 1994. {``{Determining Relative Sea-Level Change from Salt-Marsh Foraminifera and Plant Zones on the Coast of Maine, U.S.A.}''} \emph{Journal of Coastal Research} 10 (4): 990--1009.

\leavevmode\vadjust pre{\hypertarget{Gehrels2020}{}}%
Gehrels, W. R., S. Dangendorf, N. L. M. Barlow, M. H. Saher, A. J. Long, P. L. Woodworth, C. G. Piecuch, and K. Berk. 2020. {``{A Preindustrial Sea Level Rise Hotspot Along the Atlantic Coast of North America}.''} \emph{Geophysical Research Letters} 47 (4). https://doi.org/\url{https://doi.org/10.1029/2019GL085814}.

\leavevmode\vadjust pre{\hypertarget{gelman2013bayesian}{}}%
Gelman, Andrew, John B Carlin, Hal S Stern, David B Dunson, Aki Vehtari, and Donald B Rubin. 2013. \emph{Bayesian Data Analysis}. CRC press.

\leavevmode\vadjust pre{\hypertarget{Gelman1992}{}}%
Gelman, Andrew, and Donald B. Rubin. 1992. {``Inference from Iterative Simulation Using Multiple Sequences.''} \emph{Statistical Science} 7 (4): 457--72. \url{http://www.jstor.org/stable/2246093}.

\leavevmode\vadjust pre{\hypertarget{Gerlach2017}{}}%
Gerlach, Matthew J., Simon E. Engelhart, Andrew C. Kemp, Ryan P. Moyer, Joseph M. Smoak, Christopher E. Bernhardt, and Niamh Cahill. 2017. {``{Reconstructing Common Era relative sea-level change on the Gulf Coast of Florida}.''} \emph{Marine Geology} 390: 254--69. https://doi.org/\url{https://doi.org/10.1016/j.margeo.2017.07.001}.

\leavevmode\vadjust pre{\hypertarget{Gornitz2009}{}}%
Gornitz, Vivien. 2009. {``Paleoclimate Proxies, an Introduction.''} In \emph{Encyclopedia of Paleoclimatology and Ancient Environments}, 716--21. Springer Netherlands.

\leavevmode\vadjust pre{\hypertarget{Gregory2019}{}}%
Gregory, Jonathan M., Stephen M. Griffies, Chris W. Hughes, Jason A. Lowe, John A. Church, Ichiro Fukimori, Natalya Gomez, et al. 2019. {``{Concepts and Terminology for Sea Level: Mean, Variability and Change, Both Local and Global}.''} \emph{Surveys in Geophysics} 40 (6): 1251--89.

\leavevmode\vadjust pre{\hypertarget{Grinsted2015}{}}%
Grinsted, Aslak. 2015. {``{Projected Change---Sea Level}.''} \emph{Second Assessment of Climate Change for Baltic Sea Basin}, 253--63.

\leavevmode\vadjust pre{\hypertarget{Hawkes2016}{}}%
Hawkes, Andrea D., Andrew C. Kemp, Jeffrey P. Donnelly, Benjamin P. Horton, W. Richard Peltier, Niamh Cahill, David F. Hill, Erica Ashe, and Clark R. Alexander. 2016. {``{Relative sea-level change in northeastern Florida (USA) during the last 8.0ka}.''} \emph{Quaternary Science Reviews} 142: 90--101. https://doi.org/\url{https://doi.org/10.1016/j.quascirev.2016.04.016}.

\leavevmode\vadjust pre{\hypertarget{Hogarth2020}{}}%
Hogarth, P., C. W. Hughes, S. D. P. Williams, and C. Wilson. 2020. {``Improved and Extended Tide Gauge Records for the British Isles Leading to More Consistent Estimates of Sea Level Rise and Acceleration Since 1958.''} \emph{Progress in Oceanography} 184: 102333. https://doi.org/\url{https://doi.org/10.1016/j.pocean.2020.102333}.

\leavevmode\vadjust pre{\hypertarget{Holgate_PSMSL2013}{}}%
Holgate, Simon J., Andrew Matthews, Philip L. Woodworth, Lesley J. Rickards, Mark E. Tamisiea, Elizabeth Bradshaw, Peter R. Foden, Kathleen M. Gordon, Svetlana Jevrejeva, and Jeff Pugh. 2013. {``{New Data Systems and Products at the Permanent Service for Mean Sea Level}.''} \emph{Journal of Coastal Research} 29 (3): 493--504. \url{https://doi.org/10.2112/JCOASTRES-D-12-00175.1}.

\leavevmode\vadjust pre{\hypertarget{Holsclaw2013}{}}%
Holsclaw, T., B. Sansó, H. K. H. Lee Lee, K. Heitmann, S. Habib, D. Higdon, and U. Alam. 2013. {``Gaussian Process Modeling of Derivative Curves.''} \emph{Technometrics} 55 (1): 57--67. \url{http://www.jstor.org/stable/24587388}.

\leavevmode\vadjust pre{\hypertarget{Horton2018}{}}%
Horton, Benjamin P., Robert E. Kopp, Andra J. Garner, Carling C. Hay, Nicole S. Khan, Keven Roy, and Timothy A. Shaw. 2018. {``{Mapping Sea-Level Change in Time, Space, and Probability}.''} \emph{Annual Review of Environment and Resources} 43 (1): 481--521. \url{https://doi.org/10.1146/annurev-environ-102017-025826}.

\leavevmode\vadjust pre{\hypertarget{Kemp2014}{}}%
Kemp, Andrew C, Christopher E Bernhardt, Benjamin P Horton, Robert E Kopp, Christopher H Vane, W Richard Peltier, Andrea D Hawkes, Jeffrey P Donnelly, Andrew C Parnell, and Niamh Cahill. 2014. {``{Late Holocene sea- and land-level change on the U.S. southeastern Atlantic coast}.''} \emph{Marine Geology} 357: 90--100. https://doi.org/\url{https://doi.org/10.1016/j.margeo.2014.07.010}.

\leavevmode\vadjust pre{\hypertarget{Kemp2015}{}}%
Kemp, Andrew C, Andrea D Hawkes, Jeffrey P Donnelly, Christopher H Vane, Benjamin P Horton, Troy D Hill, Shimon C Anisfeld, Andrew C Parnell, and Niamh Cahill. 2015. {``{Relative sea level change in Connecticut (USA) during the last 2200 yrs}.''} \emph{Earth and Planetary Science Letters} 428: 217--29. https://doi.org/\url{https://doi.org/10.1016/j.epsl.2015.07.034}.

\leavevmode\vadjust pre{\hypertarget{Kemp2017}{}}%
Kemp, Andrew C, Troy D Hill, Christopher H Vane, Niamh Cahill, Philip M Orton, Stefan A Talke, Andrew C Parnell, Kelsey Sanborn, and Ellen K Hartig. 2017. {``{Relative sea-level trends in New York City during the past 1500 years}.''} \emph{The Holocene} 27 (8): 1169--86. \url{https://doi.org/10.1177/0959683616683263}.

\leavevmode\vadjust pre{\hypertarget{Kemp2009}{}}%
Kemp, Andrew C, Benjamin P Horton, Stephen J Culver, D Reide Corbett, Orson van de Plassche, W Roland Gehrels, Bruce C Douglas, and Andrew C Parnell. 2009. {``{Timing and magnitude of recent accelerated sea-level rise (North Carolina, United States)}.''} \emph{Geology} 37 (11): 1035--38.

\leavevmode\vadjust pre{\hypertarget{Kemp2011}{}}%
Kemp, Andrew C, Benjamin P Horton, Jeffrey P Donnelly, Michael E Mann, Martin Vermeer, and Stefan Rahmstorf. 2011. {``Climate Related Sea-Level Variations over the Past Two Millennia.''} \emph{Proceedings of the National Academy of Sciences} 108 (27): 11017--22. \url{https://doi.org/10.1073/pnas.1015619108}.

\leavevmode\vadjust pre{\hypertarget{Kemp2013SealevelUSA}{}}%
Kemp, Andrew C, Benjamin P Horton, Christopher H Vane, Christopher E Bernhardt, D Reide Corbett, Simon E Engelhart, Shimon C Anisfeld, Andrew C Parnell, and Niamh Cahill. 2013. {``{Sea level change during the last 2500 years in New Jersey, USA}.''} \emph{Quaternary Science Reviews} 81: 90--104. \url{https://doi.org/10.1016/j.quascirev.2013.09.024}.

\leavevmode\vadjust pre{\hypertarget{Kemp2015_SLhandbook}{}}%
Kemp, Andrew C., and Richard J. Telford. 2015. {``Transfer Functions: Handbook of Sea‐level Research.''} In \emph{Handbook of Sea‐level Research}, 470--99. John Wiley \& Sons, Ltd. https://doi.org/\url{https://doi.org/10.1002/9781118452547.ch31}.

\leavevmode\vadjust pre{\hypertarget{Kemp2018}{}}%
Kemp, Andrew C, Alexander J Wright, Robin J Edwards, Robert L Barnett, Matthew J Brain, Robert E Kopp, Niamh Cahill, et al. 2018. {``{Relative sea-level change in Newfoundland, Canada during the past 3000 years}.''} \emph{Quaternary Science Reviews} 201: 89--110. https://doi.org/\url{https://doi.org/10.1016/j.quascirev.2018.10.012}.

\leavevmode\vadjust pre{\hypertarget{Khan2022}{}}%
Khan, Nicole S., Erica Ashe, Ryan P. Moyer, Andrew C. Kemp, Simon E. Engelhart, Matthew J. Brain, Lauren T. Toth, et al. 2022. {``{Relative sea-level change in South Florida during the past 5000 years}.''} \emph{Global and Planetary Change} 216: 103902. https://doi.org/\url{https://doi.org/10.1016/j.gloplacha.2022.103902}.

\leavevmode\vadjust pre{\hypertarget{Khan2015}{}}%
Khan, Nicole S., Erica Ashe, Timothy A. Shaw, Matteo Vacchi, Jennifer Walker, W. R. Peltier, Robert E. Kopp, and Benjamin P. Horton. 2015. {``Holocene Relative Sea-Level Changes from Near-, Intermediate-, and Far-Field Locations.''} \emph{Current Climate Change Reports} 1 (4): 247--62.

\leavevmode\vadjust pre{\hypertarget{Kirby2023}{}}%
Kirby, Jason R, Ed Garrett, and W Roland Gehrels. 2023. {``Holocene Relative Sea-Level Changes in Northwest Ireland: An Empirical Test for Glacial Isostatic Adjustment Models.''} \emph{The Holocene}.

\leavevmode\vadjust pre{\hypertarget{Kopp2013}{}}%
Kopp, Robert E. 2013. {``{Does the mid-Atlantic United States sea level acceleration hot spot reflect ocean dynamic variability?}''} \emph{Geophysical Research Letters} 40 (15): 3981--85. \url{https://doi.org/10.1002/GRL.50781}.

\leavevmode\vadjust pre{\hypertarget{Kopp2016}{}}%
Kopp, Robert E., Andrew C. Kemp, Klaus Bittermann, Benjamin P. Horton, Jeffrey P. Donnelly, Roland W. Gehrels, Carling C. Hay, Jerry X. Mitrovica, Eric D. Morrow, and Stefan Rahmstorf. 2016. {``{Temperature-driven global sea-level variability in the Common Era}.''} \emph{Proceedings of the National Academy of Sciences of the United States of America} 113 (11): E1434--41. \url{https://doi.org/10.1073/pnas.1517056113}.

\leavevmode\vadjust pre{\hypertarget{Kopp2009}{}}%
Kopp, Robert E., Frederik J. Simons, Jerry X. Mitrovica, Adam C. Maloof, and Michael Oppenheimer. 2009. {``\href{https://www.ncbi.nlm.nih.gov/pubmed/20016591}{{Probabilistic assessment of sea level during the last interglacial stage}}.''} \emph{Nature} 462 (7275): 863--67.

\leavevmode\vadjust pre{\hypertarget{Marshall2015_SLhandbook}{}}%
Marshall, Wil. 2015. {``Chronohorizons: Handbook of Sea‐level Research.''} In \emph{Handbook of Sea‐level Research}, 373--85. John Wiley \& Sons, Ltd. https://doi.org/\url{https://doi.org/10.1002/9781118452547.ch25}.

\leavevmode\vadjust pre{\hypertarget{McHutchon2011}{}}%
McHutchon, Andrew, and Carl Edward Rasmussen. 2011. {``{Gaussian Process training with input noise}.''} \emph{Advances in Neural Information Processing Systems 24: 25th Annual Conference on Neural Information Processing Systems 2011, NIPS 2011}, 1--9.

\leavevmode\vadjust pre{\hypertarget{Meltzner2017}{}}%
Meltzner, Aron J., Adam D. Switzer, Benjamin P. Horton, Erica Ashe, Qiang Qiu, David F. Hill, Sarah L. Bradley, et al. 2017. {``{Half-metre sea-level fluctuations on centennial timescales from mid-Holocene corals of Southeast Asia}.''} \emph{Nature Communications} 8 (1): 14387. \url{https://doi.org/10.1038/ncomms14387}.

\leavevmode\vadjust pre{\hypertarget{Peltier2004}{}}%
Peltier, W. R. 2004. {``{Global Glacial Isostasy and the Surface of the Ice-Age Earth: The ICE-5G (VM2) Model and GRACE}.''} \emph{Annual Review of Earth and Planetary Sciences} 32: 111--49.

\leavevmode\vadjust pre{\hypertarget{plummer2003jags}{}}%
Plummer, Martyn. 2003. {``{JAGS: A program for analysis of Bayesian graphical models using Gibbs sampling.}''} \emph{Proceedings of the 3rd International Workshop on Distributed Statistical Computing, TUWien} 124.

\leavevmode\vadjust pre{\hypertarget{plummer2016rjags}{}}%
Plummer, Martyn, Alexey Stukalov, and Matt Denwood. 2016. {``{rjags: Bayesian graphical models using MCMC}.''} \emph{R Package Version} 4 (6).

\leavevmode\vadjust pre{\hypertarget{pugh_woodworth_2014b}{}}%
Pugh, David, and Philip Woodworth. 2014. {``Tidal Forces: Sea-Level Science: Understanding Tides, Surges, Tsunamis and Mean Sea-Level Changes.''} In \emph{Sea-Level Science: Understanding Tides, Surges, Tsunamis and Mean Sea-Level Changes}, 36--59. Cambridge University Press. \url{https://doi.org/10.1017/CBO9781139235778.006}.

\leavevmode\vadjust pre{\hypertarget{Rasmussen2006}{}}%
Rasmussen, C E, and C K I Williams. 2006. {``{Gaussian Processes for Machine Learning}.''} MIT Press.

\leavevmode\vadjust pre{\hypertarget{Shaw2018}{}}%
Shaw, Timothy A., Andrew J. Plater, Jason R. Kirby, Keven Roy, Simon Holgate, Pero Tutman, Niamh Cahill, and Benjamin P. Horton. 2018. {``{Tectonic influences on late Holocene relative sea levels from the central-eastern Adriatic coast of Croatia}.''} \emph{Quaternary Science Reviews} 200: 262--75. https://doi.org/\url{https://doi.org/10.1016/j.quascirev.2018.09.015}.

\leavevmode\vadjust pre{\hypertarget{Shennan2002}{}}%
Shennan, Ian, and Ben Horton. 2002. {``{Holocene land- and sea-level changes in Great Britain}.''} \emph{{Journal of Quaternary Science}} 17 (5-6): 511--26.

\leavevmode\vadjust pre{\hypertarget{Shennan2015_Handbook}{}}%
Shennan, Ian, Antony J. Long, and Benjamin P. Horton. 2015. {``Handbook of Sea‐level Research.''} \emph{John Wiley \& Sons, Ltd}.

\leavevmode\vadjust pre{\hypertarget{simpson2018modelling}{}}%
Simpson, Gavin L. 2018. {``Modelling Palaeoecological Time Series Using Generalised Additive Models.''} \emph{Frontiers in Ecology and Evolution} 6: 149.

\leavevmode\vadjust pre{\hypertarget{Stearns2017}{}}%
Stearns, Rachel B., and Simon E. Engelhart. 2017. {``{A High-Resolution Reconstruction of Late-Holocene Relative Sea Level in Rhode Island, USA}.''} \emph{ProQuest Dissertations and Theses}. University of Rhode Island.

\leavevmode\vadjust pre{\hypertarget{Stearns2023}{}}%
Stearns, Rachel B., Simon E. Engelhart, Andrew C. Kemp, Troy D. Hill, Matthew J. Brain, and D. Reide Corbett. 2023. {``{Within-region replication of late Holocene relative sea-level change: An example from southern New England, United States}.''} \emph{Quaternary Science Reviews} 300: 107868. https://doi.org/\url{https://doi.org/10.1016/j.quascirev.2022.107868}.

\leavevmode\vadjust pre{\hypertarget{Upton2023noisy}{}}%
Upton, Maeve, Andrew Parnell, Andrew Kemp, Erica Ashe, Gerard McCarthy, and Niamh Cahill. 2023. {``A Noisy-Input Generalised Additive Model for Relative Sea-Level Change Along the Atlantic Coast of North America.''} \emph{arXiv Preprint arXiv:2301.09556}.

\leavevmode\vadjust pre{\hypertarget{Walker2021}{}}%
Walker, Jennifer S., Robert E. Kopp, Timothy A. Shaw, Niamh Cahill, Nicole S. Khan, Donald C. Barber, Erica L. Ashe, et al. 2021. {``{Common Era sea-level budgets along the U.S. Atlantic coast}.''} \emph{Nature Communications} 12 (1): 1841. \url{https://doi.org/10.1038/s41467-021-22079-2}.

\leavevmode\vadjust pre{\hypertarget{Whitehouse2018}{}}%
Whitehouse, Pippa L. 2018. {``{Glacial isostatic adjustment modelling: historical perspectives, recent advances, and future directions}.''} \emph{Earth Surf. Dynam} 6: 401--29.

\leavevmode\vadjust pre{\hypertarget{Wickham2016}{}}%
Wickham, Hadley. 2016. \emph{Ggplot2: Elegant Graphics for Data Analysis}. Springer-Verlag New York. \url{https://ggplot2.tidyverse.org}.

\leavevmode\vadjust pre{\hypertarget{Wood2006a}{}}%
Wood, Simon N. 2006. {``{Low-Rank Scale-Invariant Tensor Product Smooths for Generalized Additive Mixed Models}.''} \emph{Biometrics} 62 (4): 1025--36.

\leavevmode\vadjust pre{\hypertarget{wood_2017}{}}%
---------. 2017a. \emph{{Generalized additive models: an introduction with R}}. CRC Press.

\leavevmode\vadjust pre{\hypertarget{Wood2017pspline}{}}%
---------. 2017b. {``P-Splines with Derivative Based Penalties and Tensor Product Smoothing of Unevenly Distributed Data.''} \emph{Statistics and Computing} 27 (4): 985--89.

\leavevmode\vadjust pre{\hypertarget{Woodworth2003}{}}%
Woodworth, P. L., and R. Player. 2003. {``{The Permanent Service for Mean Sea Level: An update to the 21st century}.''} \emph{Journal of Coastal Research} 19 (March): 287--95.

